Winning on the Merits: The Joint Effects of Content and Style on Debate Outcomes

Debate and deliberation play essential roles in politics and government, but most models presume that debates are won mainly via superior style or agenda control. Ideally, however, debates would be won on the merits, as a function of which side has the stronger arguments. We propose a predictive model of debate that estimates the effects of linguistic features and the latent persuasive strengths of different topics, as well as the interactions between the two. Using a dataset of 118 Oxford-style debates, our model's combination of content (as latent topics) and style (as linguistic features) allows us to predict audience-adjudicated winners with 74% accuracy, significantly outperforming linguistic features alone (66%). Our model finds that winning sides employ stronger arguments, and allows us to identify the linguistic features associated with strong or weak arguments.

==> argextraction.tex <==
Our topic detection and argument segmentation model is extended from Hidden Topic Markov Model (HTMM) ~\cite{gruber2007hidden}.

==> intro-example.tex <==
\begin{figure}[thbp]
	{\fontsize{9}{10}\selectfont
    \setlength{\tabcolsep}{0.6mm}
    \hspace{-2mm}
    \begin{tabular}{|p{82mm}|}
    \hline
    
    \underline{\textbf{Motion}}: {\it The U.S. should let in 100,000 Syrian refugees} \\
	$\bullet$ Debater 1 (Pro): 
	I lived in New York for two years. I'm shocked by the number of people on the streets. I walk my kids to school every morning. I'm shocked by how many people are on the streets. I don't think those -- you should ask the refugees to pay the price of sorting out those people. I think America can deal with its own social problems at home while spending, frankly, a minuscule amount of money, relatively speaking.
	\\
	$\bullet$ Debater 2 (Con): 
	They're not going to zip codes that can afford it. They're going to zip codes that have the lowest cost housing, already high unemployment rates, struggling schools. And these communities have no say in how many, what kind, or when refugees will be placed in their community. And it is  --    these refugees are not coming with an increase in federal grants or any other programs to help them shoulder the cost. \\
	$\bullet$ Debater 3 (Pro): 	
	So, here's another reality. Their idea of giving more money to Jordan, to Turkey, to Lebanon to pay for refugees -- you know what the reality is? Those countries don't want more refugees. Let me say that again. Those countries don't want more refugees. [This is a topic shift] ...
	 What I would also say though is America is a land of opportunity.  In the case of Iraqis, according to HHS, Health and Human Services statistics, 13, 1-3 percent of Iraqis in 2009 depended only on their own income to live. Everybody else, the other 87 percent, depended to some extent or another on public assistance. However, four years later, which is the last year of data for HHS, the number had gone from 13 percent to 40 percent. And the conclusion of the analysis was over time Iraqi refugees become less and less dependent on public assistance. ...
     
    \\  
    \hline
    \end{tabular}
    }
\caption{Sample arguments from debate on``Syrian refugee resettlement in U.S." The snippet focuses on resettlement effect for local communities, which is likely to be a topic that is favorable for side con. Here debater 1 (pro) and 2 (con) tend to use more emotional language, but debater 2 makes a more compelling argument. Debater 3 first talks something off-topic, and then tries to throw in numbers, however still fails to earn credit.}
\label{fig:example_intro}
\end{figure}

